Topics in Matrix Sampling Algorithms

We study three fundamental problems of Linear Algebra, lying in the heart of various Machine Learning applications, namely: 1)"Low-rank Column-based Matrix Approximation". We are given a matrix A and a target rank k. The goal is to select a subset of columns of A and, by using only these columns, compute a rank k approximation to A that is as good as the rank k approximation that would have been obtained by using all the columns; 2) "Coreset Construction in Least-Squares Regression". We are given a matrix A and a vector b. Consider the (over-constrained) least-squares problem of minimizing ||Ax-b||, over all vectors x in D. The domain D represents the constraints on the solution and can be arbitrary. The goal is to select a subset of the rows of A and b and, by using only these rows, find a solution vector that is as good as the solution vector that would have been obtained by using all the rows; 3) "Feature Selection in K-means Clustering". We are given a set of points described with respect to a large number of features. The goal is to select a subset of the features and, by using only this subset, obtain a k-partition of the points that is as good as the partition that would have been obtained by using all the features. We present novel algorithms for all three problems mentioned above. Our results can be viewed as follow-up research to a line of work known as "Matrix Sampling Algorithms". [Frieze, Kanna, Vempala, 1998] presented the first such algorithm for the Low-rank Matrix Approximation problem. Since then, such algorithms have been developed for several other problems, e.g. Graph Sparsification and Linear Equation Solving. Our contributions to this line of research are: (i) improved algorithms for Low-rank Matrix Approximation and Regression (ii) algorithms for a new problem domain (K-means Clustering).

==> rpibib.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                                 %
%%                           BIBLIOGRAPHY                          %
%%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%This method produces a numbered bibliography where the numbers
%%correspond to the \cite commands in the text. See the LaTeX manual.
%%
%\specialhead{LITERATURE CITED}
%\begin{singlespace}
%\begin{thebibliography}{99}
%\bibitem{thisbook} This is the first item in the Bibliography.
%Let's make it very long so it takes more than one line.
%Let's make it very long so it takes more than one line.
%Let's make it very long so it takes more than one line.
%Let's make it very long so it takes more than one line.
%\bibitem{anotherbook} The second item in the Bibliography.
%\bibitem{yetanotherbook} Another item in the Bibliography.
%\end{thebibliography}
%\end{singlespace}
%
%%This is an alternative method.  It's a simple unnumbered bibliography
%%with hanging indentation.
%%
%\specialhead{BIBLIOGRAPHY}
%\begin{singlespace}
%\bibentry This is the first item in the Bibliography.
%Let's make it very long so it takes more than one line.
%Let's make it very long so it takes more than one line.
%Let's make it very long so it takes more than one line.
%Let's make it very long so it takes more than one line.
%Let's make it very long so it takes more than one line.
%\bibentry The second item in the Bibliography.
%\bibentry Another item in the Bibliography.
%
%\end{singlespace}
%
%
%% Note that, if you wish, you can use BibTeX to create your bibliography
%% from a database. See section 5.6.2 of Memo RPI.110 for information.
%%%% Local Variables:
%%%% mode: latex
%%%% TeX-master: t
%%%% End:

% I use this but I put it in the main .tex file for simplicity. 
\specialhead{BIBLIOGRAPHY}
\begin{singlespace}
\bibliographystyle{abbrv}
\bibliography{RPI_BIB}
\end{singlespace}

